The Featureless HST/WFC3 Transmission Spectrum of the Rocky Exoplanet GJ 1132b: No Evidence For A Cloud-Free Primordial Atmosphere and Constraints on Starspot Contamination

Orbiting a M dwarf 12 pc away, the transiting exoplanet GJ 1132b is a prime target for transmission spectroscopy. With a mass of 1.7 Earth masses and radius of 1.1 Earth radii, GJ 1132b's bulk density indicates that this planet is rocky. Yet with an equilibrium temperature of 580 K, GJ 1132b may still retain some semblance of an atmosphere. Understanding whether this atmosphere exists and its composition will be vital for understanding how the atmospheres of terrestrial planets orbiting M dwarfs evolve. We observe five transits of GJ 1132b with the Wide Field Camera 3 (WFC3) on the Hubble Space Telescope (HST). We find a featureless transmission spectrum from 1.1--1.7 microns, ruling out cloud-free atmospheres with metallicities <300x Solar with >4.8$\sigma$ confidence. We combine our WFC3 results with transit depths from TESS and archival broadband and spectroscopic observations to find a featureless spectrum from 0.7--4.5 microns. GJ 1132b has a high mean molecular weight atmosphere, possesses a high-altitude aerosol layer, or has effectively no atmosphere. Higher precision observations are required to differentiate between these possibilities. We explore the impact of hot and cold starspots on the observed transmission spectrum GJ 1132b, quantifying the amplitude of spot-induced transit depth features. Using a simple Poisson model we estimate spot temperature contrasts, spot covering fractions, and spot sizes for GJ 1132. These limits, and the modeling framework, may be useful for future observations of GJ 1132b or other planets transiting similarly inactive M dwarfs.

==> draft_edits.tex <==
If our Solar System terrestrial planets are any indicator, rocky exoplanets likely possess a diverse population of atmospheres. Some may possess primary atmospheres enriched in hydrogen or helium while others may have undergone significant atmospheric evolution with various sources and sinks from stellar radiation and surface interactions \citep[e.g][]{segura.ozone.2003,grenfell.atmosphere.2007,hu.photochemistry.2012,luger.abiotic.2015,schaefer.gj1132b,kite.atm.loss.2020}. Characterizing these terrestrial atmospheres will be crucial towards understanding the formation, evolution, and potential habitability of these rocky worlds.

Of particular interest for atmospheric characterization are the rocky planets orbiting nearby bright M dwarfs. The smaller stellar radii of these stars translate directly into larger transit depths for Earth-sized planets passing in front of them \citep{winn.transit.review}. Moreover, these systems tend to be compact, with the expected habitable zone to be within 0.2 AU of the star \citep{kopparapu.habitable.zone}. As the probability of a transit is inversely proportional to the semi-major axis, TESS alone is expected to discover hundreds of transiting planets orbiting M dwarfs over the mission's lifetime \citep{barclay.tess,ballard.tess}. Indeed most super-Earth and Earth-sized planets amenable for transmission spectroscopy orbit nearby bright M dwarfs \citep[e.g.][]{bertathompson.et.al.2015,trappist.1.discovery,dittmann.et.al.2017,tess.2019,tess.2019.2}.

One notable planet for atmospheric study is the Earth-sized rocky planet, GJ 1132b. Discovered with the MEarth survey, this 1.13 $\pm$ 0.056 R$_{\oplus}$ and 1.66 $\pm$ 0.23 M$_{\oplus}$ rocky planet orbits a nearby inactive M4 dwarf \citep{bertathompson.et.al.2015,dittmann.et.al.2017,Bonfils.et.al.2018}. GJ 1132b receives 19x more insolation as Earth, implying an equilibrium temperature around 550 K (assuming uniform heat redistribution and albedo of 0) and placing it well outside of the habitable zone. Even though GJ 1132b receives more stellar flux than Mercury, it is also more massive leading to the question: Does GJ 1132b possess an atmosphere? And if so, what is its atmosphereic composition? GJ 1132b has already been targeted by multiple ground-based spectroscopic observations seeking answers to these questions \citep{southworth.et.al.2017,diamondlowe.et.al.2018}. \citet{southworth.et.al.2017} detected hints of a low metallicity atmosphere in their broadband observations; notably a deeper z-band transit 4$\sigma$ larger than the continuum. However, \citet{diamondlowe.et.al.2018} observed a featureless spectrum between 700 and 1040 nm with an average precision of 100 ppm per wavelength bin (equivalent to 1.8 scale heights assuming a H/He mean molecular weight). Based on their higher precision results, they ruled out a cloud-free atmosphere of $<$10x solar metallicity . \citet{diamondlowe.et.al.2018} also reports a smaller stellar radii (and thus smaller planetary radii) than that reported in \citet{southworth.et.al.2017}.

The broadband 4.5 $\mu$m Spitzer channel and the MEarth optical bandpass observations are inconclusive in supporting either data set though \citet{dittmann.et.al.2017} does determine a stellar radii in agreement to \citet{diamondlowe.et.al.2018} and \citet{bertathompson.et.al.2015}. \citet{dittmann.et.al.2017} also finds a smaller optical MEarth transit depth than in Spitzer; a depth supported by the optical spectrum from \citet{diamondlowe.et.al.2018}. However, the broadband optical depth from \citet{diamondlowe.et.al.2018} is larger than their spectroscopic points and is similar to the \citet{dittmann.et.al.2017} Spitzer depth. This difference alludes to an instrumental effect not an astrophysical one.

\citet{waalkes.et.al.2019} observed the Ly$\alpha$ ultraviolet transit of GJ 1132b using STIS. They place a 2$\sigma$ upper-limit of an exosphere at 7.3x the planetary radius. From this, they argue that it is unlikely that GJ 1132b possesses an extended hydrogen envelope created from a leftover primary atmosphere or from the photodissociation of water. \citet{waalkes.et.al.2019} calculate a mass-loss upper-limit of neutral hydrogen to be 0.86 x 10$&{9}$ g/s or one Earth ocean every 6 Myr.

While observational efforts were unable to resolve an atmosphere around GJ 1132b, theoretical work shows that any atmosphere of this planet has likely been greatly influenced by the extreme UV radiation and activity common to M dwarfs \citep{france.activity}. \citet{schaefer.gj1132b} specifically study the evolution of GJ 1132b's atmosphere in order to predict potential atmospheric compositions. In particular, they find that GJ 1132b would have initially required at least 5\% of its mass to be water in order to retain a present-day water-dominated atmosphere. As this is unlikely, \citet{schaefer.gj1132b} argue that the most likely outcome is a tenuous atmosphere dominated by O$_{2}$ created by the photodissociation of H$_{2}$O with most of the hydrogen and some of the oxygen atoms lost to space through hydrodynamic drag or absorption into a magma ocean. \citet{schaefer.gj1132b} briefly explore a CO$_{2}$ dominated atmosphere, but find that adding significant CO$_{2}$ will prolong a surface magma ocean. This ocean in turn will enhance atmospheric loss as it absorbs more water vapor and diassociated O$_{2}$. However, they note that further study is required on the possible carbon cycle of GJ 1132b.

We investigate the existence of an atmosphere around GJ 1132b by observing its transmission spectrum from \textit{The Hubble Space Telescope (HST)} Wide-Field Camera 3 (WFC3) between 1.1 and 1.7 microns. We achieve transit depth precisions of 40 ppm per 20 nm wavelength bins (equivalent to 0.34 scale heights assuming H/He atmosphere) over five visits. These observations enabled us to place constraints on possible atmospheric compositions while also searching for the presence of water which would provide insights into the atmospheric history of this planet. 

However, stellar activity, especially unocculted stellar spots and faculae have the potential to either mimic or mask planetary water features in the WFC3 bandpass \citep{rackham.general,zhang.trappist1}. GJ 1132, with a rotation period of 130 days is not a young active M dwarf \citep{newton.gj1132.rotation}. Constant monitoring with MEarth allude to a spot covering fraction of (NEED VALUE). \citet{dittmann.et.al.2017} note an offset between the MEarth optical and Spitzer infrared transit depths which they attribute to unocculted stellar spots. It is therefore apparent that quantifying stellar activity on GJ 1132 is necessary for correct interpretation of planetary spectra observed by both \textit{HST}/WFC3 and future instruments such as the \textit{James Webb Space Telescope (JWST)} and ELTs.

We present the \textit{HST}/WFC3 transmission spectrum of GJ 1132b collected over five different transits. We outline the observations in Section~\ref{sec:observation} and detail the analysis of the broadband and spectroscopic light curves in Section~\ref{sec:analysis}. We present the analysis of the TESS light curve of GJ 1132 in this section as well. Section~\ref{sec:discussion} discusses the transmission spectrum and the possible atmospheric compositions for GJ 1132b including a comparison to the recent WFC3 results from \citet{swain.et.al.2021}. We quantify stellar contamination in this spectrum in Section~\ref{sec:discussion} before concluding in Section~\ref{sec:conclusion}.

\section{Observations and Data Reduction}
\label{sec:observations}

We reduced each of the five WFC3 visits using the publicly available Iraclis pipeline\footnote{https://github.com/ucl-exoplanets/Iraclis}. We included a summary of the pipeline's steps here; \citet{iraclis.2016a} and \citet{iraclis.2016b} provide a full description of the pipeline's methodology. Starting with the RAW spatially scanned spectroscopic images, Iraclis performed the following: a zero-read subtraction, non-linearity correction, dark correction, gain conversion, flat fielding, sky background subtraction, and bad pixel and cosmic ray interpolation. Iraclis calculates potential horizonal and vertical shifts in the scanned spectrum over time and determines the scan length for each image by approximating a Gaussian along the sum of the rows. With the direct image of GJ 1132, wavelength is assigned and the wave dependent flat field is applied. Iraclis reports times in units of HJD which we converted to $BJD_{TDB}$ using the time utilities code provided by Jason Eastman\footnote{http://astroutils.astronomy.ohio-state.edu/time/} \citep{eastman.et.al.2012}.

We extracted the 1-D spectrum by applying a 166-pixel wide aperture along the dispersion axis and summing along the cross-dispersion axis for each wavelength. As the average scan length for each image is about 170 pixels, our slightly smaller aperture was chosen to minimize potential edge effects of the scan. However, slightly smaller and larger apertures (162 pixels and 172 pixels) had no notable improvement on the results.

Across the five visits there is less than a 0.2 pixel shift in both the x- and y-directions of the scan. A comparison of the residuals from the best-fit models to these shifts demonstrated no correlation. We therefore did not apply any correction to these small shifts. We also found no correlation with either the scan length or background values to the residuals.

GJ 1132 lies in a crowded stellar field where possible spectra overlap could occur \citep{bertathompson.et.al.2015} (CITATION?). We checked the direct images of each visit which showed no other nearby bright star in the field of view. A comparison of the average spectrum between visits demonstrated less than a 1\% flux variation across all wavelengths (Figure~\ref{fig:contamination}), leading us to conclude there is no outside contamination to the WFC3 GJ 1132b spectrum.

From the Iraclis reduced spectra, we created broadband light curves for each visit by summing the flux from 1


We present the WFC3-determined weighted average transit depths for GJ 1132b in Figure~\ref{fig:hst_metal}. We found that the planet's transmission spectrum is best explained by a flat or featureless spectrum with a $\chi^{2}_{r}$ of NEED VALUE with 21 degrees of freedom. From the weighted uncertainties, we approximated that the 1$\sigma$ precisions corresponds to NEED value scale heights for GJ 1132b assuming a H/He dominated atmosphere. We comapred our measurements to cloud-freee transmission models of varying metallicities in Figure~\ref{fig:hst_metal} and atmospheres compoesed of 100\% H$_{2}$O, CO$_{2}$, and O$_{2}$ in Figure~\ref{fig:hst_mole}. Model pressure-temperature (P-T) profiles were calculated ELIZA DO YOU MIND ADDING SOME DETAILS ABOUT THE MODEL OR I CAN CITE THE EXOTRANSMIT PAPERS FOR EASE.

From the WFC3 observations, we confidently rule out atmospheres with metallicities $<$300x solar with $>$5$\sigma$ corresponding to an atmospheric mean molecular weight of $>$8.9 amu. If we assume an atmosphere composition of part H/He and part H$_{2}$O, this mean molecular weight is comparable to a 44\% H$_{2}$O and 54\% H/He atmosphere by atomic mass. However, given GJ 1132b's equilibrium temperature of 530 K \citep{Bonfils.et.al.2018}, it is more likely that this planet possesses an atmosphere CO$_{2}$ dominated similar to Venus, a tenuous O$_{2}$ as discuseed in \citet{schaefer.gj1132b} or no atmosphere at all. Figure~\ref{fig:hst_mole} shows that we cannot rule out any of these scenarios with the current WFC3 precision. 

\subsubsection{Previous HST/WFC3 Results}
Recently two other papers have published the same HST/WFC3 data with very different results \citep{swain.et.al.2021,mugnai.et.al.2021}. \citet{swain.et.al.2021} determined a H/He-rich atmosphere with a Rayleigh scattering slope and HCN absorption indicating the presence of haze. \citet{mugnai.et.al.2021} in turn found a featureless spectrum with transit depths and uncertaintites similar to ours (Figure~\ref{fig:swain_compare}). \citet{mugnai.et.al.2021} used both the Iraclis pipeline and the NEED PIPELINE used by \citet{swain.et.al.2021}, and determined the same featureless spectrum. However, both studies use an analytical model to remove systematics. We in turn compared both their analytical ramp model and the physically motivated model RECTE in Section~\ref{sec:analysis} and found no different in transit depths. Therefore, the differing results in \citet{swain.et.al.2021} do not appear to be due to either data reduction or the systematic model. Given the similarities between our results and \citet{mugnai.et.al.2021}, we conclude that GJ 1132b does not possess an extended H/He dominated atmosphere, though future observations with higher precision is required to determine the atmospheric composition.

\subsubsection{Clouds and Hazes}
Featureless exoplanet transmission spectra are attributed to two different causes: a higher mean molecular weight atmosphere (and thus smaller scale height) or a high-altitude aerosol layer muting or blocking absorption features. While GJ 1132b's temperature and terrestrial nature suggest a higher mean molecular weight atmosphere, we cannot rule out the possibility of a lower H/He dominated atmosphere combined with clouds or hazes. We therefore retrieve the alitutde required for an aerosol layer to mute all features in the WFC3 transmission spectrum. Assuming a 1x Solar composition, we place aerosol layers at increasing altitudes until we obtain a spectrum that agrees with the data (p-value of 0.001) \citep[described in][]{libbyroberts.et.al.2020}. We find that this layer must lie at pressure levels $<$0.4 mbars in order to mute to properly mute the features of a H/He dominated atmosphere. However, using models from \citet{lopez.and.fortney.2014}, we calculate an expected H/He percentage of less than 1\% for GJ 1132b and therefore do not favor clouds/hazes as the sole cause for the WFC3 flat spectrum.

\subsubsection{Comparison with Archival Data}

We compare the WFC3 transit depths with archival data from \citet{dittmann.et.al.2017}, \citet{southworth.et.al.2017}, and \citet{diamondlowe.et.al.2018} in Figure~\ref{fig:spec_no_off}. We also include the broadband TESS point derived from Section~\ref{sec:tess_analysis}, and the updated MEarth depth of NEED VALUE (private communication with Jonathan Irwin). The inclusion of all data sets support a featureless spectrum from $\sim$0.7 - 4.5 $\mu$m (from opitcal to Spitzer's 4.5 $\mu$m channel) with a $\chi^{2}_{r}$ of NEED VALUE. We do not include  the broadband points from \citet{southworth.et.al.2017} in this calculation due to the large discrepancies between their transit depths and all other depths. 

A closer inspection of the spectroscopic points from \citet{diamondlowe.et.al.2018} shows that their depths appear smaller than the rest of the archival data. Unocculted stellar activity can alter a planet's spectrum, making the planet's transit depth appear smaller at shorter wavelengths than at longer ones \citep{rackham.general}. However, a closer inspection of the transit depths reported in \citet{diamondlowe.et.al.2018} shows that their broadband depth is deeper than any of their spectroscopic depths while also being statistically the same as the depths derived from WFC3 (Figure~\ref{fig:diamond-lowe}). As it is harder to quantify systematics within the lower signal-to-noise spectroscopic bins, the overall effect may have contributed to the smaller transit depth. We conclude that the difference between the \citet{diamondlowe.et.al.2018} spectroscopic points and the WFC3 points are due to instrumental not astrophysical effects.

We applied an offset to \citet{diamondlowe.et.al.2018} calculated so that the weighted average transit depth of their spectroscopic points is equal to their broadband transit depth (Figure~\ref{fig:spec_off}). We recalculated a goodness-of-fit for a flat spectrum and determined a $\chi^{2}_{r}$ of NEED VALUE. The combined data sets improve the atmospheric constraints by ruling out atmospheres with metallicities $<$300x solar with $>$6$\sigma$ confidence. 


hdiamondlowe: More thoughts on this: If the back-and-forth over GJ 1132b's atmosphere has taught us anything it's that there is a fundamental misunderstanding of what we mean when we say we are looking for H/He atmospheres. It might be good to clarify that for planets with terrestrial radii and masses we know from their bulk densities alone that they do not possess >1% of their masses in H/He envelopes. Rather, we are interested in the case where these worlds have accreted and maintained <0.1% of their masses in H/He, which could be enough to be detectable in transmission via trace species with spectral features, but not enough to detect in the planet's a bulk density. The Owen paper I mentioned goes into this nicely.





==> future_work.tex <==
Benjamin Rackham: If we should suspect the parameters to be strictly wavelength-independent, then perhaps they could be estimated more robustly in a joint fit (i.e., using a single set of RECTE parameters while allowing R_p/R_s to vary for each spectroscopic light curve).
(for the spectroscopic fits)

A referee once told me I should use the Kipping re-parameterization of the quadratic LD law. I don't think it's absolutely necessary but something to be aware of: https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.2152K/abstract
Fitting for limb darkening coefficients for TESS and potentially WFC3

We used the Gaia-determined stellar effective temperature of 3630 K \citep{gaia.et.al.2018b} in calculating the limb-darkening coefficients. - We just need to re-run all this with a different limb darkening version prior to submission


hdiamondlowe: Ooh, it's been a while but lemme try: I believe Eliza's code assumes a "grey" opacity (i.e., a single opacity value, not varying with wavelength). A double-grey profile means that there is one opacity for short-wave (optical) radiation that can be trapped in the planet's atmosphere and another opacity for long-wave (IR) radiation that can escape to space. Having the double-grey opacity can better capture the ability of an atmosphere to trap heat at one wavelength and let it escape at another wavelength, while also letting a bunch of computationally expensive radiative transfer calculations collapse to simpler ODEs. (I think.)


Changing HST inflation: I agree that inflating to the time of a full datapoint is overkill, but that we also probably shouldn't trust them down to the ridiculous few second precision either. A good in-between (again for the resubmission) would be to inflate the errors so that the WFC3 data themselves are consistent with the period and T0 (that is, that the reduced chisq of the five times around the straight line is 1).

Re-run visits to check for convergence: Also: how can the chisqrd be better than the case where you let a/R and i float? (it is chisqrd/dof but the denominator change is very small) when comparing the two versions...this happens on two visits

Fix table 2 to include more sig figs

==> old_revisions.tex <==
With the upcoming launch of the James Webb Space Telescope (JWST), we will be equipped to study the atmospheres of rocky terrestrial planets. If our Solar System terrestrial planets are any indicator, rocky exoplanets likely posses a diverse population of atmospheres. Some may possess primary atmospheres enriched in hydrogen or helium while others may have undergone significant atmospheric evolution with various sources and sinks both from the stellar radiation and surface interactions (CITATION suggestions?). Characterizing these terrestrial atmospheres will be crucial towards understanding the formation, evolution, and potential habitability of these rocky worlds.

Of particular interest for atmospheric characterization are the rocky planets orbiting nearby bright M dwarfs. The smaller stellar radii of these stars translate directly into larger transit depths for Earth-sized planets passing in front of them \citep{winn.transit.review}. Moreover, these systems tend to be compact, with the expected habitable zone to be within 0.2 AU of the star \citep{kasting.habitable.zone}. As the probability of transit is inversely proportional to semi-major axis, we expect to discover a large number of transiting planets around M dwarfs \citep{winn.transit.review}; a feature that is supported by the Kepler mission \citep{dressing.mdwarf.occurence}. Indeed most super-Earth and Earth-sized planets amenable for transmission spectroscopy orbit nearby bright M dwarfs (CITATION?).

One notable planet for atmospheric study is the Earth-sized rocky planet, GJ 1132b. Discovered with the MEarth survey, this 1.1 R$_{\oplus}$ and 1.6 M$_{\oplus}$ rocky planet orbits a nearby (12 pc) inactive M4 dwarf \citep{bertathompson.et.al.2015}. With an equilibrium temperature around 500 K, this planet received 19x more insolation as Earth placing it well outside of the habitable zone. However, it is still possible that GJ 1132b may possess an atmosphere and has already been targeted by multiple ground-based atmospheric studies. \citet{diamondlowe.et.al.2018} observed a featureless spectrum between 700 to 1040 nm with an average precision of 100 ppm per wavelength bin (precision equivalent to 1.8 scale heights assuming H/He mean molecular weight). Based on these results, they rule out a cloud-free atmosphere of $<$10x solar metallicity. On the other hand, observations in \citet{southworth.et.al.2017} hint at a low metallicity atmosphere. They observe a deeper z-band transit 4$\sigma$ larger than the continuum which could indicate a strong water absorption feature. However, they also determine a larger stellar radii (and thus larger planetary radii) than that reported in \citet{diamondlowe.et.al.2018} and \citet{bertathompson.et.al.2015}.

The broadband 4.5 $\mu$m Spitzer observations and the MEarth optical bandpasses are inconclusive in supporting either data set though \citet{dittmann.et.al.2017} does determine a stellar radii in agreement to \citet{diamondlowe.et.al.2018} and \citet{bertathompson.et.al.2015}. \citet{dittmann.et.al.2017} also determines a smaller optical MEarth transit depth than in Spitzer, a depth also supported by the optical spectrum from \citet{diamondlowe.et.al.2018}. However, the broadband optical depth from \citet{diamondlowe.et.al.2018} is larger than their spectroscopic points and is similar to the \citet{dittmann.et.al.2017} Spitzer point. We will discuss this detail further in Section (NEED NUMBER).

\cite{waalkes.et.al.2019} observed the Ly$\alpha$ ultraviolet transit of GJ 1132b using STIS determining a 2$\sigma$ upper-limit of an exosphere of 7.3x the planetary radius. From this, they argue that it is unlikely that GJ 1132b possesses an extended hydrogen envelope created from the photodissociation of water. \citet{waalkes.et.al.2019} calculate a mass-loss limit of netural hydrogen to be 0.86 x 10$^{9}$ g/s or one Earth ocean every 6 Myr.

Based on these many studies of GJ 1132b questions still remain as to: 1. Does GJ 1132b have an atmosphere? 2. If it does, is it primordial or secondary in nature? M dwarfs likely sculpt the atmospheres of their planets, more so than other stars due to their extreme UV-to-bolometric flux ratios (CITATIONS see WAALKES paper). The extreme activity of these stars may strip the atmospheres of nearby rocky planets (CITE SEGURA and YOUNGBLOOD papers). \citet{schaefer.gj1132b} specifically study the evolution of an atmosphere around GJ 1132b in order to predict possible atmospheric compositions. In particular, they find that GJ 1132b would have initially required at least 5\% of its mass to be water in order to retain a present-day water-dominated atmophsere. As this is unlikely, \citet{schaefer.gj1132b} argue that the most likely outcome is a tenuous atmosphere dominated by O$_{2}$ created by the photodissociation of H$_{2}$O with most of the hydrogen and oxygen atoms lost to space through hydrodynamic drag or absorption into a magma ocean. Discovering substantial amounts of atmospheric water would indicate either the existence of a large H$_{2}$ envelope or an unusually low XUV flux from GJ 1132 earlier in the star's lifetime. Motivated by GJ 1132b's Venus-like temperature, \citet{schaefer.gj1132b} briefly explore a CO$_{2}$ dominated atmosphere, but find that adding CO$_{2}$ in the atmosphere will prolong a magma ocean that could enhance atmospheric loss by absorbing more water vapor and diassociated O$_{2}$. However, they note that further study is required on the possible carbon cycle on GJ 1132b.

We investigate the existence of an atmosphere around GJ 1132b by observing its transmission spectrum from \textit{The Hubble Space Telescope (HST)} Wide-Field Camera 3 (WFC3) between 1.1 and 1.7 microns. We achieve transit depth precisions of 40 ppm per 20nm wavelength bin (0.34 scale heights assuming H/He atmosphere) over 5 visits. This enabled us to place constraints on possible atmospheric compositions while also searching for water which could provide insights into the UV-flux history of this planet.

However, stellar activity, especially unocculted stellar spots and faculae have the potential to either mimic or mask planetary water features in the WFC3 bandpass \citep{zhang.trappist1,rackham.general}. While this is notably an issue in the shorter optical bandpasses, \citet{rackham.gj1214} demonstrates the ability to constrain and quantify stellar activity of GJ 1214 when combining optical spectra to WFC3 spectra. 

GJ 1132, with a rotation period of 130 days (Newton paper) is not an active M dwarf. Constant monitoring with MEarth allude to spot covering fractions of (need value) (cite Newton paper again?). Even with little activity, \citet{dittmann.et.al.2017} note discrepancy between MEarth optical and Spitzer broadband transit depths which are likely caused by unocculted stellar spots. It is therefore apparent that quantifying stellar activity on GJ 1132 and M dwarfs in general will be necessary for correct interpretation of planetary spectra observed by both HST/WFC3 and future JWST.

We present the HST/WFC3 transmission spectrum of GJ 1132b collected over 5 different transits. We outline the observations in Section (NEED SECTION NUMBER) and detail the analysis of the broadband and spectroscopic light curves in Section (NEED SECTION NUMBER). We also present the analysis of the TESS light curve of GJ 1132 in this section. Section (NEED SECTION NUMBER) discusses possible atmospheric compositions for GJ 1132b as well as quantifies the stellar contamination within the HST/WFC3 spectrum and archival optical observations. We conclude in Section (NEED SECTION NUMBER). 

We reduced each of the WFC3 visits using the publicly available Iraclis pipeline\footnote{https://github.com/ucl-exoplanets/Iraclis}. \citet{iraclis.2016a} and \citet{iraclis.2016b} provide a full explanation of the pipeline's methodology; we provide a summary of it here. Starting with the RAW spatially scanned spectroscopic images, Iraclis performed the following steps: a zero-read subtraction, non-linearity correction, dark correction, gain conversion, flat fielding, sky background subtraction, and bad pixel and cosmic ray interpolation. Iraclis then calculated potential horizontal and vertical shifts in the scanned spectrum over time and determined a scan length for each image by approximating a Gaussian along the sum of the rows. With the direct image of GJ 1132, wavelength was assigned and the wave dependent flat field was applied. Iraclis reports times in units of HJD which we converted to $BJD_{TDB}$ using the time utilities code provided by Jason Eastman\footnote{http://astroutils.astronomy.ohio-state.edu/time/} \citep{eastman.et.al.2012}.

We extracted the 1-D spectrum by applying a 166-pixel wide aperture along the dispersion axis and summing along the cross-dispersion axis for each wavelength. As the average scan length for each image is about 170 pixels, our slightly smaller aperture was chosen to minimize possible edge effects of the scan. However, we found that slightly larger and smaller apertures (172 pixels and 162 pixels) had no notable improvement on the results.

Across the five visits there is less than a 0.2 pixel shift in both the x and y directions of the scan. A comparison of the residuals from the best-fit models (discussed in Section~\ref{bblc}) to that of these shifts demonstrated no correlation. We therefore did not apply any correction to these small shifts. We also found no correlation with either the scan length or background values to the residuals.

GJ 1132 lies in a crowded stellar field where possible spectra overlap could occur (CITATION?). We checked the direct images for each visit which showed no other bright star in the field a view. Furthermore, a comparison of the average spectrum between visits demonstrated less than a 1\% flux variation across all wavelengths (Figure~\ref{fig:contamination}) leading us to conclude there is no outside contamination to the GJ 1132 spectrum.


We calculated the autocorrelation length for each parameter and found that they are significantly small (GET NUMBER FOR THIS) and therefore the walkers converged.


This result contrasts with that of \citet{swain.et.al.2021} who use this same data set to determine a H/He-rich atmosphere with a Rayleigh scattering slope. A comparison of their spectroscopic transit depths compared to this analysis are plotted in Figure~\ref{fig:swain_compare}. We find smaller error bars in this work while also being more consistent with a flat or featureless line. It appears the discrepancy between the two studies falls at shorter wavelengths, though we are unsure as to the cause of this difference.


\subsection{Clouds and Hazes}

Featureless exoplanet transmission spectra can be attributed to two different causes: a higher mean molecular weight atmosphere (and thus smaller scale height) or a high-altitude aerosol layer muting or blocking absorption features. As discussed in the previous section, GJ 1132b's featureless WFC3 spectrum is likely due to a higher mean molecular weight atmosphere than our precision can detect. However, we cannot rule out the possibility of a lower H/He dominated atmosphere combined with clouds or hazes. We test the altitude required for an aerosol layer to mute all features in the GJ 1132b spectrum. Assuming a 1x Solar composition, we place aerosol layers at higher and higher altitudes until we obtain a flat spectrum that agrees with our data with a p-value of 0.001 (CHECK THIS) (see \citet{libbyroberts.et.al.2020} for a full description of this process). 

Assuming a gray opacity aerosol layer, we require this layer to lie at pressure levels less than 0.4 mbars. These pressures are similar to the top of the cloud deck in Venus's atmosphere (CITATION). The difference lies in our results requiring a H/He dominated atmopshere compared to the CO$_{2}$ enriched one on Venus. That said, it is difficult to justify how GJ 1132b manages to maintain a H/He dominated atmopshere at its mass, size, and insolation over the course of its $>$5 Gyr lifetime \citep{bertathompson.et.al.2015}. Using \citet{lopez.and.fortney.2014} models, we calculate an expected H/He percentage of less than 1\% for GJ 1132b and therefore do not favor clouds/hazes as the sole cause behind the WFC3 flat spectrum of this planet.

A comparison of these WFC3 results with other archival data supports a higher mean molecular weight atmosphere as well, though with noted discrepancy. Figure~\ref{fig:spec} plots the transmission spectra of GJ 1132b from \citet{dittmann.et.al.2017}, \citet{southworth.et.al.2017}, and \citet{diamondlowe.et.al.2018}, as well as the updated MEarth point of NEED NUMBER (private communication with Jonathan Irwin) and this work's WFC3 and TESS transit depths. The top panel plots these points as they are reported with varying atmospheric metallicities for comparison. The bottom panel includes an offset for the \citet{southworth.et.al.2017} and \citet{diamondlowe.et.al.2018} points so they are on par with the WFC3 spectrum. The most notable difference between the two panels are the optical points from \citet{diamondlowe.et.al.2018} which possess a notable smaller transit depth compared to all other points. It is possible that this smaller transit depth is due to stellar contamination, as was observed in the optical spectrum for GJ 1214b \citep{rackham.gj1214}. We will explore this possibility further in Section (NEED SECTION). However, the broadband depth reported in \citet{diamondlowe.et.al.2018} is (NEED VALUE), similar to all other transit depths except \citet{southworth.et.al.2017}. We therefore recommend caution when comparing these data sets as instrumental and systematic noise may be the cause of this discrepancy. As for the differences in the transit depths from \citet{southworth.et.al.2017}, they conclude very different stellar and planetary radii for this system and we are hesitant to draw any conclusions from a direct comparison with their work.



\begin{figure}
\centering

\begin{subfigure}{.8\textwidth}
\centering
\includegraphics[width=.8\textwidth]{total_spectrum_no_off.pdf} 
\label{fig:spec_no_off}
\end{subfigure}
\vspace{.01cm}
\begin{subfigure}{.8\textwidth}
\centering
\includegraphics[width=.8\textwidth]{total_spectrum_off.pdf} 
\label{fig:spec_off}
\end{subfigure}

\caption{A comparison of this work's WFC3 spectrum (black points) and broadband TESS transit depth (dark red) with that of \citet{diamondlowe.et.al.2018} (dark blue points), the 4.5 $\mu$m {\it Spitzer} point from \citet{dittmann.et.al.2017} (dark purple), \citet{southworth.et.al.2017} broadband depths (light purple), \citet{swain.et.al.2021} (light blue), and the updated MEarth depth (light green). Top panel assumes no offset between each data set and plots the points as the depths are reported. Bottom panel assumes offsets for the optical \citet{diamondlowe.et.al.2018} and \citet{southworth.et.al.2017} points such that their medium transit depth is the same as WFC3. We calculate best-fit statistics for each atmospheric model by only using our WFC3 and TESS depths along with \citet{dittmann.et.al.2017} and \citet{diamondlowe.et.al.2018}. The top panel suggests that the optical spectrum from \citet{diamondlowe.et.al.2018} has a smaller transit depth than the other studies which may be due to astrophysical noise such as star spots or instrumental effects. Correcting for this offset shows support for a featureless spectrum for GJ 1132b.}
\label{fig:spec}
\end{figure}


 \citet{dittmann.et.al.2017} finds a smaller optical MEarth transit depth than in {\it Spitzer}; a depth supported by the optical spectrum from \citet{diamondlowe.et.al.2018}. However, the broadband optical depth from \citet{diamondlowe.et.al.2018} is larger than their spectroscopic points and is similar to the \citet{dittmann.et.al.2017} {\it Spitzer} depth. This difference alludes to an instrumental effect not an astrophysical one.
 
 We achieve transit depth precision of 40 ppm in 20 nm wavelength bins (equivalent to 0.34 scale heights assuming H/He atmosphere) over five visits.
 
 
%\citet{mugnai.et.al.2021} used both the {\tt iraclis} and the {\tt CASCADe} pipelines determining the same featureless spectrum. However, both studies apply an analytical model to remove systematics. We in turn compared both their analytical ramp model and the physically motivated model {\tt RECTE} in Section~\ref{sec:analysis} and found no different in transit depths. Therefore, the deviating results in \citet{swain.et.al.2021} do not appear to be due to either data reduction or the systematic model. Given the similarities between our results and \citet{mugnai.et.al.2021}, we conclude that GJ 1132b does not possess an extended H/He dominated atmosphere, though future observations with higher precision is required to determine the atmospheric composition.

Using the {\it TESS} light curve, we place additional constraints on other transiting bodies. We place an upper 3$\sigma$ limit of 1.84 R$_{\oplus}$ on the radius of GJ 1132c assuming the planet transits. 

Orbiting a M dwarf only 12 pc away, the transiting exoplanet GJ 1132b is a prime target for transmission spectroscopy. With a mass of 1.7 M$_{\oplus}$ and radius of 1.1 R$_{\oplus}$, GJ 1132b's bulk density indicates that this planet is rocky. GJ 1132b's equilibrium temperature of 580 K suggests that this planet may be able to retain some semblance of an atmosphere (either thick or tenuous). Understanding whether this atmosphere exists as well as its composition would provide vital information for understanding how the atmospheres of terrestrial planets orbiting M dwarfs evolve. We observe five transits of GJ 1132b with the Wide Field Camera 3 (WFC3) on the {\it Hubble Space Telescope (HST)}. We find a featureless transmission spectrum for GJ 1132b from 1.1 to 1.7 $\mu$m, ruling out cloud-free atmospheres with metallicities $<$300$\times$ Solar by volume with $>$4.8$\sigma$ confidence. We combine our WFC3 results with the broadband transit depth we measured from {\it TESS}, an updated MEarth transit depth, and archival optical and {\it Spitzer} depths, demonstrating a featureless spectrum from 0.7--4.5 $\mu$m for GJ 1132b. The additional data enables us to rule out a cloud-free H/He dominated atmosphere at $>$5.6$\sigma$. GJ 1132b therefore has a high mean molecular weight atmosphere, possesses a high-altitude aerosol layer, or has no atmosphere at all. Higher precision observations are required to differentiate between these possibilities. We also explore the impact of starspots on GJ 1132 (both cold and hot) on the observed transmission spectrum of the planet. Incorporating five years of photometric monitoring from the MEarth Observatory, we quantify the amplitude of spot-induced features that could potentially be confused with the planet's transmission spectrum. Using a simple Poisson model for the distribution of spots across the stellar disk, we make estimates of spot temperature contrasts, spot covering fractions, and spot sizes for GJ 1132. These starspot limits, and the modeling framework, may be useful for future observations of GJ 1132b or other planets transiting similarly inactive mid-to-late M dwarfs. 


==> widetab.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllrrrrrrll}
\tablecaption{Observable Characteristics of 
Galactic/Magellanic Cloud novae with X-ray observations\label{chartable}}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Name} & \colhead{V$_{max}$} & 
\colhead{Date} & \colhead{t$_2$} & 
\colhead{FWHM} & \colhead{E(B-V)} & 
\colhead{N$_H$} & \colhead{Period} & 
\colhead{D} & \colhead{Dust?} & \colhead{RN?} \\ 
\colhead{} & \colhead{(mag)} & \colhead{(JD)} & \colhead{(d)} & 
\colhead{(km s$^{-1}$)} & \colhead{(mag)} & \colhead{(cm$^{-2}$)} &
\colhead{(d)} & \colhead{(kpc)} & \colhead{} & \colhead{}
} 
\startdata
CI Aql & 8.83 (1) & 2451665.5 (1) & 32 (2) & 2300 (3) & 0.8$\pm0.2$ (4) & 1.2e+22 & 0.62 (4) & 6.25$\pm5$ (4) & N & Y \\
{\bf CSS081007} & \nodata & 2454596.5 & \nodata & \nodata & 0.146 & 1.1e+21 & 1.77 (5) & 4.45$\pm1.95$ (6) & \nodata & \nodata \\
GQ Mus & 7.2 (7) & 2445352.5 (7) & 18 (7) & 1000 (8) & 0.45 (9) & 3.8e+21  & 0.059375 (10) & 4.8$\pm1$ (9) & N (7) & \nodata \\
IM Nor & 7.84 (11) & 2452289 (2) & 50 (2) & 1150 (12) & 0.8$\pm0.2$ (4) & 8e+21 & 0.102 (13) & 4.25$\pm3.4$ (4) & N & Y \\
{\bf KT Eri} & 5.42 (14) & 2455150.17 (14) & 6.6 (14) & 3000 (15) & 0.08 (15) & 5.5e+20 & \nodata & 6.5 (15) & N & M \\
{\bf LMC 1995} & 10.7 (16) & 2449778.5 (16) & 15$\pm2$ (17) & \nodata & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
LMC 2000 & 11.45 (18) & 2451737.5 (18) & 9$\pm2$ (19) & 1700 (20) & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
{\bf LMC 2005} & 11.5 (21) & 2453700.5 (21) & 63 (22) & 900 (23) & 0.15 (203) & 1e+21 & \nodata & 50  & M (24) & \nodata \\
{\bf LMC 2009a} & 10.6 (25) & 2454867.5 (25) & 4$\pm1$  & 3900 (25) & 0.15 (203)  & 5.7e+20 & 1.19 (26) & 50 & N & Y \\
{\bf SMC 2005} & 10.4 (27) & 2453588.5 (27) & \nodata & 3200 (28) & \nodata & 5e+20  & \nodata & 61 & \nodata & \nodata \\
{\bf QY Mus} & 8.1 (29) & 2454739.90 (29) & 60:  & \nodata & 0.71 (30) & 4.2e+21  & \nodata & \nodata & M & \nodata \\
{\bf RS Oph} & 4.5 (31) & 2453779.44 (14) & 7.9 (14) & 3930 (31) & 0.73 (32) & 2.25e+21 & 456 (33) & 1.6$\pm0.3$ (33) & N (34) & Y \\
{\bf U Sco} & 8.05 (35) & 2455224.94 (35) & 1.2 (36) & 7600 (37) & 0.2$\pm0.1$ (4) & 1.2e+21 & 1.23056 (36) & 12$\pm2$ (4) & N & Y \\
{\bf V1047 Cen} & 8.5 (38) & 2453614.5 (39) & 6 (40) & 840 (38) & \nodata & 1.4e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V1065 Cen} & 8.2 (41) & 2454123.5 (41) & 11 (42) & 2700 (43) & 0.5$\pm0.1$ (42) & 3.75e+21 & \nodata & 9.05$\pm2.8$ (42) & Y (42) & \nodata \\
V1187 Sco & 7.4 (44) & 2453220.5 (44) & 7: (45) & 3000 (44) & 1.56 (44) & 8.0e+21 & \nodata & 4.9$\pm0.5$ (44) & N & \nodata \\
{\bf V1188 Sco} & 8.7 (46) & 2453577.5 (46) & 7 (40) & 1730 (47) & \nodata & 5.0e+21  & \nodata & 7.5 (39) & \nodata & \nodata \\
{\bf V1213 Cen} & 8.53 (48) & 2454959.5 (48) & 11$\pm2$ (49) & 2300 (50) & 2.07 (30) & 1.0e+22 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1280 Sco} & 3.79 (51) & 2454147.65 (14) & 21 (52) & 640 (53) & 0.36 (54) & 1.6e+21  & \nodata & 1.6$\pm0.4$ (54) & Y (54) & \nodata \\
{\bf V1281 Sco} & 8.8 (55) & 2454152.21 (55) & 15:& 1800 (56) & 0.7 (57) & 3.2e+21 & \nodata & \nodata & N & \nodata \\
{\bf V1309 Sco} & 7.1 (58) & 2454714.5 (58) & 23$\pm2$ (59) & 670 (60) & 1.2 (30) & 4.0e+21 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1494 Aql} & 3.8 (61) & 2451515.5 (61) & 6.6$\pm0.5$ (61) & 1200 (62) & 0.6 (63) & 3.6e+21  & 0.13467 (64) & 1.6$\pm0.1$ (63) & N & \nodata \\
{\bf V1663 Aql} & 10.5 (65) & 2453531.5 (65) & 17 (66) & 1900 (67) & 2: (68) & 1.6e+22  & \nodata & 8.9$\pm3.6$ (69) & N & \nodata \\
V1974 Cyg & 4.3 (70) & 2448654.5 (70) & 17 (71) & 2000 (19) & 0.36$\pm0.04$ (71) & 2.7e+21  & 0.081263 (70) & 1.8$\pm0.1$ (72) & N & \nodata \\
{\bf V2361 Cyg} & 9.3 (73) & 2453412.5 (73) & 6 (40) & 3200 (74) & 1.2: (75) & 7.0e+21 & \nodata & \nodata & Y (40) & \nodata \\
{\bf V2362 Cyg} & 7.8 (76) & 2453831.5 (76) & 9 (77) & 1850 (78) & 0.575$\pm0.015$ (79) & 4.4e+21  & 0.06577 (80) & 7.75$\pm3$ (77) & Y (81) & \nodata \\
{\bf V2467 Cyg} & 6.7 (82) & 2454176.27 (82) & 7 (83) & 950 (82) & 1.5 (84) & 1.4e+22  & 0.159 (85) & 3.1$\pm0.5$ (86) & M (87) & \nodata \\
{\bf V2468 Cyg} & 7.4 (88) & 2454534.2 (88) & 10: & 1000 (88) & 0.77 (89) & 1.0e+22  & 0.242 (90) & \nodata & N & \nodata \\
{\bf V2491 Cyg} & 7.54 (91) & 2454567.86 (91) & 4.6 (92) & 4860 (93) & 0.43 (94) & 4.7e+21  & 0.09580: (95) & 10.5 (96) & N & M \\
V2487 Oph & 9.5 (97) & 2450979.5 (97) & 6.3 (98) & 10000 (98) & 0.38$\pm0.08$ (98) & 2.0e+21 & \nodata & 27.5$\pm3$ (99) & N (100) & Y (101) \\
{\bf V2540 Oph} & 8.5 (102) & 2452295.5 (102) & \nodata & \nodata & \nodata & 2.3e+21 & 0.284781 (103) & 5.2$\pm0.8$ (103) & N & \nodata \\
V2575 Oph & 11.1 (104) & 2453778.8 (104) & 20: & 560 (104) & 1.4 (105) & 3.3e+21 & \nodata & \nodata & N (105) & \nodata \\
{\bf V2576 Oph} & 9.2 (106) & 2453832.5 (106) & 8: & 1470 (106) & 0.25 (107) & 2.6e+21  & \nodata & \nodata & N & \nodata \\
{\bf V2615 Oph} & 8.52 (108) & 2454187.5 (108) & 26.5 (108) & 800 (109) & 0.9 (108) & 3.1e+21  & \nodata & 3.7$\pm0.2$ (108) & Y (110) & \nodata \\
{\bf V2670 Oph} & 9.9 (111) & 2454613.11 (111) & 15: & 600 (112) & 1.3: (113) & 2.9e+21  & \nodata & \nodata & N (114) & \nodata \\
{\bf V2671 Oph} & 11.1 (115) & 2454617.5 (115) & 8: & 1210 (116) & 2.0 (117) & 3.3e+21  & \nodata & \nodata & M (117) & \nodata \\
{\bf V2672 Oph} & 10.0 (118) & 2455060.02 (118) & 2.3 (119) & 8000 (118) & 1.6$\pm0.1$ (119) & 4.0e+21  & \nodata & 19$\pm2$ (119) & \nodata & M \\
V351 Pup & 6.5 (120) & 2448617.5 (120) & 16 (121) & \nodata & 0.72$\pm0.1$ (122) & 6.2e+21 & 0.1182 (123) & 2.7$\pm0.7$ (122) & N & \nodata \\
{\bf V382 Nor} & 8.9 (124) & 2453447.5 (124) & 12 (40) & 1850 (23) & \nodata & 1.7e+22 & \nodata & \nodata & \nodata & \nodata \\
V382 Vel & 2.85 (125) & 2451320.5 (125) & 4.5 (126) & 2400 (126) & 0.05: (126) & 3.4e+21  & 0.146126 (127) & 1.68$\pm0.3$ (126) & N & \nodata \\
{\bf V407 Cyg} & 6.8 (128) & 2455266.314 (128) & 5.9 (129) & 2760 (129) & 0.5$\pm0.05$ (130) & 8.8e+21 & 15595 (131) & 2.7 (131) & \nodata & Y \\
{\bf V458 Vul} & 8.24 (132) & 2454322.39 (132) & 7 (133) & 1750 (134) & 0.6 (135) & 3.6e+21 & 0.06812255 (136) & 8.5$\pm1.8$ (133) & N (135) & \nodata \\
{\bf V459 Vul} & 7.57 (137) & 2454461.5 (137) & 18 (138) & 910 (139) & 1.0 (140) & 5.5e+21  & \nodata & 3.65$\pm1.35$ (138) & Y (140) & \nodata \\
V4633 Sgr & 7.8 (141) & 2450895.5 (141) & 19$\pm3$ (142) & 1700 (143) & 0.21 (142) & 1.4e+21  & 0.125576 (144) & 8.9$\pm2.5$ (142) & N & \nodata \\
{\bf V4643 Sgr} & 8.07 (145) & 2451965.867 (145) & 4.8 (146) & 4700 (147) & 1.67 (148) & 1.4e+22 & \nodata & 3 (148) & N & \nodata \\
{\bf V4743 Sgr} & 5.0 (149) & 2452537.5 (149) & 9 (150) & 2400 (149) & 0.25 (151) & 1.2e+21 & 0.281 (152) & 3.9$\pm0.3$ (151) & N & \nodata \\
{\bf V4745 Sgr} & 7.41 (153) & 2452747.5 (153) & 8.6 (154) & 1600 (155) & 0.1 (154) & 9.0e+20  & 0.20782 (156) & 14$\pm5$ (154) & \nodata & \nodata \\
{\bf V476 Sct} & 10.3 (157) & 2453643.5 (157) & 15 (158) & \nodata & 1.9 (158) & 1.2e+22  & \nodata & 4$\pm1$ (158) & M (159) & \nodata \\
{\bf V477 Sct} & 9.8 (160) & 2453655.5 (160) & 3 (160) & 2900 (161) & 1.2: (162) & 4e+21  & \nodata & \nodata & M (163) & \nodata \\
{\bf V5114 Sgr} & 8.38 (164) & 2453081.5 (164) & 11 (165) & 2000 (23) & \nodata & 1.5e+21  & \nodata & 7.7$\pm0.7$ (165) & N (166) & \nodata \\
{\bf V5115 Sgr} & 7.7 (167) & 2453459.5 (167) & 7 (40) & 1300 (168) & 0.53 (169) & 2.3e+21  & \nodata & \nodata & N (169) & \nodata \\
{\bf V5116 Sgr} & 8.15 (170) & 2453556.91 (170) & 6.5 (171) & 970 (172) & 0.25 (173) & 1.5e+21 & 0.1238 (171) & 11$\pm3$ (173) & N (174) & \nodata \\
{\bf V5558 Sgr} & 6.53 (175) & 2454291.5 (175) & 125 (176) & 1000 (177) & 0.80 (178) & 1.6e+22  & \nodata & 1.3$\pm0.3$ (176) & N (179) & \nodata \\
{\bf V5579 Sgr} & 5.56 (180) & 2454579.62 (180) & 7: & 1500 (23) & 1.2 (181) & 3.3e+21 & \nodata & \nodata & Y (181) & \nodata \\
{\bf V5583 Sgr} & 7.43 (182) & 2455051.07 (182) & 5: & 2300 (182) & 0.39 (30) & 2.0e+21 & \nodata & 10.5 & \nodata & \nodata \\
{\bf V574 Pup} & 6.93 (183) & 2453332.22 (183) & 13 (184) & 2800 (184) & 0.5$\pm0.1$  & 6.2e+21 & \nodata & 6.5$\pm1$  & M (185) & \nodata \\
{\bf V597 Pup} & 7.0 (186) & 2454418.75 (186) & 3: & 1800 (187) & 0.3 (188) & 5.0e+21  & 0.11119 (189) & \nodata & N (188) & \nodata \\
{\bf V598 Pup} & 3.46 (14) & 2454257.79 (14) & 9$\pm1$ (190) & \nodata & 0.16 (190) & 1.4e+21 & \nodata & 2.95$\pm0.8$ (190) & \nodata & \nodata \\
{\bf V679 Car} & 7.55 (191) & 2454797.77 (191) & 20: & \nodata & \nodata & 1.3e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V723 Cas} & 7.1 (192) & 2450069.0 (192) & 263 (2) & 600 (193) & 0.5 (194) & 2.35e+21  & 0.69 (195) & 3.86$\pm0.23$ (196) & N & \nodata \\
V838 Her & 5 (197) & 2448340.5 (197) & 2 (198) & \nodata & 0.5$\pm0.1$ (198) & 2.6e+21  & 0.2975 (199) & 3$\pm1$ (198) & Y (200) & \nodata \\
{\bf XMMSL1 J06} & 12 (201) & 2453643.5 (202) & 8$\pm2$ (202) & \nodata & 0.15 (203) & 8.7e+20 & \nodata & 50 & \nodata & \nodata \\
\enddata
\end{deluxetable}
\end{longrotatetable}

